ConfigFix: Interactive Configuration Conflict Resolution for the Linux Kernel

Highly configurable systems are highly complex systems, with the Linux kernel arguably being one of the most well-known ones. Since 2007, it has been a frequent target of the research community, conducting empirical studies and building dedicated methods and tools for analyzing, configuring, testing, optimizing, and maintaining the kernel in the light of its vast configuration space. However, despite a large body of work, mainly bug fixes that were the result of such research made it back into the kernel's source tree. Unfortunately, Linux users still struggle with kernel configuration and resolving configuration conflicts, since the kernel largely lacks automated support. Additionally, there are technical and community requirements for supporting automated conflict resolution in the kernel, such as, for example, using a pure C-based solution that uses only compatible third-party libraries (if any). With the aim of contributing back to the Linux community, we present CONFIGFIX, a tooling that we integrated with the kernel configurator, that is purely implemented in C, and that is finally a working solution able to produce fixes for configuration conflicts. In this experience report, we describe our experiences ranging over a decade of building upon the large body of work from research on the Linux kernel configuration mechanisms as well as how we designed and realized CONFIGFIX while adhering to the Linux kernel's community requirements and standards. While CONFIGFIX helps Linux kernel users obtaining their desired configuration, the sound semantic abstraction we implement provides the basis for many of the above techniques supporting kernel configuration, helping researchers and kernel developers.

==> kconfigexample.tex <==
\section{Kconfig Example}

\begin{lstlisting}[caption={Menu-configuration in Kconfig },label={lst:kconfigsnippet},language=kconfig,float=t]
menu "Architectures"

menu "Misc"
config EX
		bool "Example option"
endmenu

config X86
		bool "X86 architecture"

config 64BIT
		bool "64 bit support"
		depends on X86

config ARM
		bool "ARM architecture"

endmenu
\end{lstlisting}

\begin{figure}[b]
\centering
	\includegraphics[width=.6\columnwidth]{fig/xconfig_menu.png}
	\caption{The example from \lstref{lst:kconfigsnippet} rendered in \xconfig}
	\label{fig:xconfig_menu}
\end{figure}


==> rangefix.tex <==
\section{RangeFix}
\label{sec:rangefix}
\looseness=-1

When dealing with conflicts in a constraint satisfaction problem \cite{csp} such as Boolean satisfiability problems, an important question is how to resolve conflicts. Given an assignment of values which violates constraints, the goal is often not to just find \textit{any} assignment that satisfies all constraints, but rather one that requires as few changes as possible.\\
Different conflict-resolution algorithms had been developed, though they all had certain drawbacks. They either produced only one solution, too many solutions or they only offered limited support for non-Boolean constraints. \citeauthor{rangefix} proposed the algorithm \textit{RangeFix} in the paper \textquote{Range Fixes: Interactive Error Resolution for Software Configuration} \cite{rangefix} and the algorithm was designed to mitigate the aforementioned problems by offering a range of values for certain options as well as support for non-Boolean constraints and options. As a result, properties for RangeFix include correctness, a maximality of ranges and a minimality of variables to be changed.\\
\textit{How does the algorithm work?} RangeFix achieves generating a list of fixes for the problem in three stages. In the first stage all minimal sets of variables, which have to be changed, are generated. These minimal sets are called diagnoses. In the stages 2 and 3 the new values for each variable in a diagnosis are calculated. The algorithm is best illustrated with an example.\\
\textit{Example:} The tuple $(V,e,c)$ is defined as a \textit{constraint violation}, where $V$ is a set of variables, $e$ a configuration with a value defined for each variable and $c$ a set of constraints which is violated. The goal is to find a new configuration $e'$, such that $c$ is satisfied. We define our set of variables $V$ as:
$$\{m: Boolean, a: Integer, b: Integer\}$$
A set of constraints is defined as:
$$(m \rightarrow a > 10)\ \land (\neg m \rightarrow b > 10)\ \land (a < b)$$
Finally, a configuration $e$ with values for the three variables is required:
$\{m:= True, a:= 6 , b:= 5\}$. Unfortunately, this configuration violates several constraints. To be precise both the first and the third constraint are violated.\\
RangeFix generates the diagnoses during the first stage by using constraint solvers' ability to return unsatisfiable cores. During each iteration in the first step, one constraint from an unsatisfiable core is removed and the diagnoses are extended until no more unsatisfiable core is found. Applying this to the example yields the following two diagnoses: $\{m, b\}$ and $\{a, b\}$. At this point, we know that we need to change either $\{m, b\}$ or $\{a, b\}$ in order to resolve the conflict.\\
The stages 2 and 3 are subsequently performed together for each diagnosis. First, all unchanged variables are replaced by their current values during stage 2. Finally in stage 3, the violated constraints are minimised with the help of heuristic rules and split into minimal clauses in order to generate the fixes. That leads to the following two fixes for the conflict:
\begin{itemize}
	\item $[m:= False, b: b > 10]$
	\item $[(a,b): a > 10 \land a < b]$
\end{itemize}

